Nanostars planarity modulates the elasticity of DNA hydrogels

In analogy with classic rigidity problems of networks and frames, the elastic properties of hydrogels made of DNA nanostars (DNAns) are expected to strongly depend on the precise geometry of their building blocks. However, it is currently not possible to determine DNAns shape experimentally. Computational coarse-grained models that can retain the correct geometry of DNA nanostars and account for the bulk properties observed in recent experiments could provide missing insights. In this study, we perform metadynamics simulations to obtain the preferred configuration of three-armed DNA nanostars simulated with the oxDNA model. Based on these results we introduce a coarse-grained computational model of nanostars that can self assemble into complex three dimensional percolating networks. We compare two systems with different designs, in which either planar or non-planar nanostars are used. Structural and network analysis reveal completely different features for the two cases, leading to two contrasting elastic properties. The mobility of molecules is larger in the non-planar case, which is consistent with a lower viscosity measured from Green-Kubo simulations in equilibrium. To the best of our knowledge, this is the first work connecting the geometry of DNAns with the bulk rheological properties of DNA hydrogels and may inform the design of future DNA based materials.

==> intermediate1.tex <==



==> intermediate2.tex <==


